Auto-MAP: A DQN Framework for Exploring Distributed Execution Plans for DNN Workloads

The last decade has witnessed growth in the computational requirements for training deep neural networks. Current approaches (e.g., data/model parallelism, pipeline parallelism) parallelize training tasks onto multiple devices. However, these approaches always rely on specific deep learning frameworks and requires elaborate manual design, which make it difficult to maintain and share between different type of models. In this paper, we propose Auto-MAP, a framework for exploring distributed execution plans for DNN workloads, which can automatically discovering fast parallelization strategies through reinforcement learning on IR level of deep learning models. Efficient exploration remains a major challenge for reinforcement learning. We leverage DQN with task-specific pruning strategies to help efficiently explore the search space including optimized strategies. Our evaluation shows that Auto-MAP can find the optimal solution in two hours, while achieving better throughput on several NLP and convolution models.

==> background/background.tex <==
\section{Background}
\begin{figure}[H]
    \includegraphics[width=0.45\textwidth]{background/type-of-parallelism.png}
    \caption{
     Typical types of parallelism.
    }
    \label{fig:dapple}
\end{figure}
\subsection{Data Parallelism}

\subsection{Model Parallelism}

\subsection{Pipeline Parallelism}
Pipeline Parallelism has been recently proposed to train DNN in a pipelined manner. GPipe\cite{huang2019gpipe} explores synchronous pipeline approach to train large models with limited GPU memory. PipeDream\cite{harlap2018pipedream} explores the hybrid approach of data and pipeline parallelism for asynchronous training.
% \cite{guan2019xpipe,geng2019elasticpipe,chen2018efficient} make further optimization based on PipeDream.
Pal et al. \cite{pal2019optimizing} evaluated the hybrid approach without thorough study.
% Some researchers have been seeking for the optimal placement strategy
% to assign operations in a DNN to different devices\cite{mirhoseini2017device, gu2019tiresias, wang2019supporting} to further improve system efficiency.
\subsection{Rainbow DQN}
Reinforcement learning (RL) is a general framework where agents learn to perform actions in an environment so as to maximize a reward. The two main components are the environment, which represents the problem to be solved, and the agent, which represents the learning algorithm.
DQN\cite{mnih2015human} is a RL algorithm that combines Q-Learning with deep neural networks to let RL work for complex, high-dimensional environments, like video games, or robotics.
% Double DQN\cite{van2016deep} Corrects the stock DQN algorithm’s tendency to sometimes overestimate the values tied to specific actions.
Rainbow DQN\cite{hessel2018rainbow} is an off-policy deep reinforcement
learning algorithm that is the state-of-the-art technique in
the field of reinforcement learning


